Product Kernel Interpolation for Scalable Gaussian Processes

Recent work shows that inference for Gaussian processes can be performed efficiently using iterative methods that rely only on matrix-vector multiplications (MVMs). Structured Kernel Interpolation (SKI) exploits these techniques by deriving approximate kernels with very fast MVMs. Unfortunately, such strategies suffer badly from the curse of dimensionality. We develop a new technique for MVM based learning that exploits product kernel structure. We demonstrate that this technique is broadly applicable, resulting in linear rather than exponential runtime with dimension for SKI, as well as state-of-the-art asymptotic complexity for multi-task GPs.

==> method.tex <==
%!TEX root=../main.tex
\section{Method}

In this paper, we will use the running example of personalized forecasting predictions
when formulating the problem and our methods.
%However, what we present is sufficiently
%general and can be applied to a variety of multi-task problems.
%
Assume that we would like to make forecasting predictions for $\numpeople$ people. In healthcare
applications, we might have access to previous patient measurements, and we would like
to predict these measurements at future times.
Each person $p \in 1, \ldots, \numpeople$ is represented by a collection of
$T_p$ data points $\{ \x_p, \y_p \}$,
where $\y_p = y^{(1)}_p, \ldots, y^{(T_p)}_p$ corresponds to previously-recorded
measurements and $\x_p = x^{(1)}_p, \ldots, x^{(T_p)}_p$ corresponds
to the times measurements were collected.
\gp{Discuss other time-dependent features?}
We do not assume that measurements were collected at evenly-spaced intervals,
nor do we assume that measurements were collected at the same time for different
patients, i.e. for people $p$ and $p'$, $\x_p \neq \x_{p'}$ and $T_p \neq T_{p'}$.

Given $\dset = \{ (\x_p, \y_p) \}_{p=1}^\numpeople$, our goal is to predict future
measurement values $\ytest_p(\xtest)$ for person $p$ at a future time $\xtest > \x_p$.
In other words, we would like to learn the predictive distribution
$\Pr{ \ytest_p(\xtest) \mid \xtest, p, \dset }$ \agw{$p(\cdot)$ rather than Pr.  It's a density
not a probability.  Possibly you don't want to overlap with $p$ for person, but perhaps use a 
different letter for that... such as `s' for subject}.
We can formulate this task \agw{formulate this objective... to avoid overloading the word task} as a multi-task regression problem. At each future time
$\xtest$, we can consider the \numpeople{} predictive tasks $\ytest_1(\xtest), \ldots,
\ytest_\numpeople(\xtest)$ -- one predictive task per person.

\subsection{Multi-task Gaussian processes}

Multi-task Gaussian process models are a natural choice for this type of forecasting
problem.
A standard Gaussian process (GP) model would assume a Gaussian process
prior over the measurements for a person $p$.
In other words, $y_p(t) \sim \GP{\mu}{k_\text{feat}}$,
where $\mu$ is a mean function (typically zero) and $k_\text{feat}$ is a
function that models the covariance between two measurements based on the inputs:
%
$$k_\text{feat} ( x^{(i)}, x^{(i')} ) = \covariance ( y_p(x^{(i)}), y_p(x^{(i')}).$$
%
Multi-task Gaussian processes extend this model by assuming a GP prior on
measurements across \emph{all} individuals. We use a covariance function $k_\text{multi}$
that augments $k_\text{feat}$ with a task-specific covariance $k_\text{task}$.
Thus $k_\text{multi}$ measures covariance across individuals $p$ and $p'$
as well as across inputs $x^{(i)}$ and $x^{(i')}$:
%
\begin{align*}
  k_\text{multi} ( [ x^{(i)}; p ], [ x^{(i')}; p'] )
  &= \covariance ( y_p(x^{(i)}), y_{p'}(x^{(i')}).
  \\
  &= k_\text{feat} ( x^{(i)} , x^{(i')} ) k_\text{task} ( p, p' ).
\end{align*}
%
$k_\text{feat}$ takes the form of a kernel function, such as the RBF kernel or the
spectral mixture kernel \cite{wilson2013gaussian}.
$k_\text{task}$ is parameterized
by a person-correlation matrix $\taskmat^\text{ppl} \in \reals^{\numpeople \times \numpeople}$ -- i.e.
$k_\text{task}(p, p') = \taskmat^\text{ppl}_{p, p'}$.
We learn the hyperparameters of $k_\text{feat}$ and the entries of $\taskmat^\text{ppl}$
by optimizing the marginal log likelihood of the data.

It is worth noting that our formulation of multi-task GPs differs slightly from the original.
\citet{bonilla2008multi} assume that inputs map to outputs for \emph{each} task.
Since we assume that inputs $x_p^i$ are unique to each person, we assume that inputs map
to outputs for a \emph{single} task. Thus we cannot formulate the covariance matrix in
terms of Kronecker products, as in \cite{bonilla2008multi}.
Under our formulation, the covariance matrix is expressed as an element-wise multiplication:
%
$$K^\text{multi} = K^\text{feat} \odot K^\text{task}.$$
%
$K^\text{feat}$ is constructed by calculating $k_\text{feat}$ on all pairs of points.
$K^\text{task}$ on the other hand is constructed using $\taskmat^\text{ppl}$ as a lookup table
 -- i.e., given tasks $p_i$ and $p_j$, $K^\text{task}_{i, j} = \taskmat^\text{ppl}_{p_i, p_j}$.
We can efficiently implement this \agw{this what?} using matrix multiplies:
%
$$K^\text{task} = \taskindmat \taskmat^\text{ppl} \taskindmat^T$$
%
where $\taskindmat \in \{0, 1\}^{n \times \numpeople}$ is a sparse index matrix
with each row $v_i$ is a one-hot encoding of task $p_i$.
%
To ensure that $K^\text{task}$ is positive semi-definite, we constrain $\taskmat^\text{ppl}$ to take
the form
%
\begin{equation}
  \taskmat^\text{ppl} = \mathbf B \mathbf B^T + \text{diag} ( \mathbf \kappa ),
  \label{eqn:taskmat_form}
\end{equation}
where $\mathbf B$ is a low-rank matrix (the rank $r$ is a hyperparameter)
and $\mathbf \kappa \in \reals^n$ is a vector.

\paragraph{Scaling with tasks.}
As $\numpeople$, the number of tasks, increases, the number of model parameters in
$\taskmat^\text{ppl}$ increases quadratically. We find empirically that learning is significantly impeded
as the number of parameters in increases. When formulating $\taskmat^\text{ppl}$ as in \eqref{eqn:taskmat_form},
the model is very sensitive to the rank of the matrix $B$.
If the rank is too small, it becomes difficult to construct as $\taskmat^\text{ppl}$ which can fully captures
correlations between people. If the rank is too large, it becomes increasingly likely that the model
overfits.
Empirically, we find that when $\numpeople$ exceeds 20, even changing the rank by 1 significantly alters
results.
While it would be possible to sweep over all possible values of rank,
or marginalizing out the parameters in $\taskmat^\text{ppl}$, the computational cost to do so may make training this
model infeasible.\agw{Actually, a prior over M seems quite reasonable here}

\subsection{Learning clusters}
To avoid parameter explosion, our goal is to reduce the dimensionality of the task-correlation
matrix.
We accomplish this by discovering \emph{latent subpopuliation clusters} in the data,
and parameterizing $k_\text{task}$ in terms of correlations between clusters rather than people.
Given $\numclusters$ clusters, we now parameterize $k_\text{task}$ by a matrix
$\taskmat^\text{c} \in \reals^{\numclusters \times \numclusters}$. If $\numclusters << \numpeople$,
then the number of parameters to learn will be significantly reduced.
We can now rewrite $K^\text{task}$ as $K^\text{task} = \taskindmat \taskmat^\text{c} \taskindmat^T$,
where $\taskindmat \in \reals^{n \times \numclusters}$ is a matrix where each row $\mathbf v_i$
represents a categorical distribution over person $p_i$'s cluster assignment.
\agw{How do you learn the clusters?}
\gp{Draw connection to parameter sharing in $\taskmat^\text{ppl}$.}

\subsection{Scaling to large datasets}


==> sections/skip.tex <==
%!TEX root=../main.tex
\section{Structured kernel interpolation for product kernels}
\label{sec:ski}
In this section, we briefly review Structured Kernel Interpolation \citep{wilson2015kernel}, a method that dramatically reduces the matrix-vector multiplication time with non-product kernels. We then discuss SKI for product kernels--which we call \emph{SKIP}--by integrating our method with SKI, thus allowing SKI to be applied to product kernels. We then provide two applications that demonstrate the greatly increased applicability of SKI.

\subsection{Structured kernel interpolation}
Structured kernel interpolation is a technique for scalable Gaussian process inference that seeks to replace a user-specified kernel $k(\x,\x')$ with an approximate kernel that leads to very fast matrix-vector multiplies with the resulting kernel matrix $\K_{\X\X}$. Assume we are given a set of $m$ \emph{inducing points} $\U$ that we will use to approximate kernel values. The underlying assumption is essentially that, if $\bu_{a}$ is very close to $\x$ and $\bu_{b}$ is very close to $\x'$, then $k(\x, \x')$ is well approximated by $k(\bu_{a}, \bu_{b})$.

Thus, instead of computing kernel values between data points directly, SKI computes kernel values between inducing points and interpolate these kernel values to approximate the true data kernel values. This leads to the approximate SKI kernel:
%
\begin{equation}\label{eq:interp_single}
    k(\x,\bz) = \bw_{\x}\K_{\U\U}\bw_{\bz}^{\top},
\end{equation}
%
where $\bw_{\x}$ is a sparse vector that contains interpolation weights. For example, when using local cubic interpolation \citep{keys1981cubic}, $\bw_{x}$ contains four nonzero elements. Applying this approximation for all data points in the training set, we see that:
\begin{equation}
  \K_{\X\X} = \W_{\X}\K_{\U\U}\W_{\X}^{\top}
\end{equation}
With arbitrary inducing points $\U$, matrix-vector multiplies with $[\W\K_{\U\U}\W^{\top}]\bv$ require $\bigo{n+m^{2}}$ time \citep{wilson2015kernel}. In one dimension, instead choosing $\U$ to be a regular grid results in $\K_{\U\U}$ being \emph{Toeplitz}. In higher dimensions, using a multi-dimensional grid resulting in $\K_{\U\U}$ being the Kronecker product of Toeplitz matrices. This results in the ability to perform matrix-vector multiplies in $\bigo{n + m \log m}$ time. Furthermore, storing $\W$ and $\K_{\U\U}$ requires $\bigo{n + m}$ space.

\subsection{Structured kernel interpolation for products}
Given a product kernel $\K=\K^{(1)}_{\X\X} \circ \cdots \circ \K^{(d)}_{\X\X}$, we apply the SKI approximation to each component as:
\begin{equation}
\K^{(i)}_{\X\X}=\W^{(i)}\K_{\U\U}\W^{(i)\top}.
\end{equation}
This immediately provides us with fast matrix-vector multiplies $\mvm{\K^{(i)}_{\X\X}}$. When using SKI approximations, the running time of our product kernel inference technique with $p$ iterations of CG becomes $\bigo{dk(n + m \log m) + k^{3}n\log d + pk^{2}n}$. The running time of SKIP is compared to that of other inference techniques in \autoref{tab:time}.

